Can Humans Identify Domains?

Textual domain is a crucial property within the Natural Language Processing (NLP) community due to its effects on downstream model performance. The concept itself is, however, loosely defined and, in practice, refers to any non-typological property, such as genre, topic, medium or style of a document. We investigate the core notion of domains via human proficiency in identifying related intrinsic textual properties, specifically the concepts of genre (communicative purpose) and topic (subject matter). We publish our annotations in *TGeGUM*: A collection of 9.1k sentences from the GUM dataset (Zeldes, 2017) with single sentence and larger context (i.e., prose) annotations for one of 11 genres (source type), and its topic/subtopic as per the Dewey Decimal library classification system (Dewey, 1979), consisting of 10/100 hierarchical topics of increased granularity. Each instance is annotated by three annotators, for a total of 32.7k annotations, allowing us to examine the level of human disagreement and the relative difficulty of each annotation task. With a Fleiss' kappa of at most 0.53 on the sentence level and 0.66 at the prose level, it is evident that despite the ubiquity of domains in NLP, there is little human consensus on how to define them. By training classifiers to perform the same task, we find that this uncertainty also extends to NLP models.

==> Figure/models.tex <==
\definecolor{deepchampagne}{rgb}{0.98, 0.84, 0.65}
\definecolor{darkgreen}{rgb}{0.0, 0.2, 0.13}
\definecolor{lightgrey}{rgb}{0.7, 0.7, 0.7}


\begin{tikzpicture}


\node (model1) [rectangle, fill, draw, lightgrey, line width=.05cm, opacity=.25, minimum width=3.4cm, minimum height=1cm] at (4.75,-1.6) {};
\node (model2) [rectangle, fill, draw, lightgrey, line width=.05cm, opacity=.25, minimum width=3.4cm, minimum height=2cm] at (4.75,-3.65) {};
\node (model3) [rectangle, fill, draw, lightgrey, line width=.05cm, opacity=.25, minimum width=3.4cm, minimum height=2cm] at (4.75,-6.2) {};
\node (model4) [rectangle, fill, draw, lightgrey, line width=.05cm, opacity=.25, minimum width=3.4cm, minimum height=1.7cm] at (1.1,-6.5) {};


\node (text) [text width=3cm, fill=white, rectangle callout,draw, rounded corners=3pt] at (2.5,3) {This is... HEY!};

\node (ann1) [] at (0,1) {\includegraphics[width=1cm]{Figure/woman-factory-worker_1f469-200d-1f3ed}};
\node (ann2) [] at (2,1) {\includegraphics[width=1cm]{Figure/man-supervillain_1f9b9-200d-2642-fe0f}};
\node (ann3) [] at (4,1) {\includegraphics[width=1cm]{Figure/woman-farmer-medium-dark-skin-tone_1f469-1f3fe-200d-1f33e}};

\draw [->] (text) -- (ann1);
\draw [->] (text) -- (ann2);
\draw [->] (text) -- (ann3);

%\draw [->] ([yshift=-.55cm]out2.south) -- (out2.south);

\node (label1) [text height=.2cm, text depth=.2cm] at (0,-.25) {Vlog};
\node (label2) [text height=.2cm, text depth=.2cm] at (2,-.25) {Vlog};
\node (label3) [text height=.2cm,text depth=.2cm] at (4,-.25) {Conversation};

\draw [->] (ann1) -- (label1);
\draw [->] (ann2) -- (label2);
\draw [->] (ann3) -- (label3);

\draw (0,-1) -- (0,-3) -- (2.5,-3);

\node (firstAmount) [rectangle, fill, deepchampagne, minimum width=.3cm, minimum height=.75cm] at (.2,-2.6) {};
\node (secondAmount) [rectangle, fill, darkgreen, minimum width=.3cm, minimum height=1.5cm] at (1.25,-2.25) {};

\node (score) [] at (-.5,-2.25) {.33};
\node (score) [] at (-.5,-1.5) {.66};
\node(anchor) [] at (1, -1) {};

\draw [->] (label1) -- (anchor);
\draw [->] (label2) -- (anchor);
\draw [->] (label3) -- (anchor);

\node (label1) [rotate=45] at (0,-3.5) {conv.};
\node (label2) [rotate=45] at (0.5, -3.5) {fiction};
\node (label3) [rotate=45] at (1,-3.5) {vlog};
\node (label4) [rotate=45] at (1.5, -3.5) {news};
\node (label5) [rotate=45] at (2,-3.5) {...};


\node (model_maj) [] at (4,-1.5) {\includegraphics[width=1cm]{Figure/robot-clipart-xl}};
\node (model_maj) [] at (4,-1) {Majority};
\node (model_maj) [] at (5.5,-1.5) {\setlength{\tabcolsep}{2pt} \begin{tabular}{ll}\includegraphics[width=.4cm]{Figure/robot_1f916} & : ``Vlog''\\ \end{tabular}};

\node (model_perlabel1) [] at (4,-3.5) {\includegraphics[width=1cm]{Figure/robot-clipart-xl}};
\node (model_maj) [] at (4.5,-2.5) {PerLabel-Regr.};
\node (model_maj) [] at (5.5,-3.75) {\setlength{\tabcolsep}{2pt} \renewcommand{\arraystretch}{.5}
\begin{tabular}{ll}
\includegraphics[width=.4cm]{Figure/robot_1f916} &: 0.33 \\
\includegraphics[width=.4cm]{Figure/robot_1f916} & : 0.0 \\
\includegraphics[width=.4cm]{Figure/robot_1f916} & : 0.66 \\
\includegraphics[width=.4cm]{Figure/robot_1f916} & : ... \\
\end{tabular}};


\node (model_perlabel1) [] at (4,-6) {\includegraphics[width=1cm]{Figure/robot-clipart-xl}};
\node (model_maj_label2) [] at (4.5,-5) {PerLabel-Clas.};
\node (model_maj) [] at (5.5,-6.25) {\setlength{\tabcolsep}{2pt} \renewcommand{\arraystretch}{.5}
\begin{tabular}{ll}
\includegraphics[width=.4cm]{Figure/robot_1f916} &: ``0.33'' \\
\includegraphics[width=.4cm]{Figure/robot_1f916} & : ``0.0'' \\
\includegraphics[width=.4cm]{Figure/robot_1f916} & : ``0.66'' \\
\includegraphics[width=.4cm]{Figure/robot_1f916} & : ... \\
\end{tabular}};

\node (model_peranno) [] at (0,-6.3) {\includegraphics[width=1cm]{Figure/robot-clipart-xl}};
\node (model_maj_label) [] at (0.5,-5.5) {PerAnno};
\node (model_maj) [] at (1.7,-6.5) {\setlength{\tabcolsep}{2pt} \renewcommand{\arraystretch}{.5}
\begin{tabular}{ll}
\includegraphics[width=.4cm]{Figure/robot_1f916} &: ``Vlog'' \\
\includegraphics[width=.4cm]{Figure/robot_1f916} & : ``Vlog'' \\
\includegraphics[width=.4cm]{Figure/robot_1f916} & : ``Conv.'' \\
\end{tabular}};


\draw [->] (label5) -- ([yshift=-.55cm]model1.west);
\draw [->] (label5) -- (model2);
\draw [->] (label5) -- (model_maj_label2.west);
\draw [->] (label4) -- (model_maj_label);


%\node (model_perlabel2) [] at (3,-5) {\includegraphics[width=1cm]{Figure/robot-clipart-xl}};

%\node (model_peranno) [] at (0,-5) {\includegraphics[width=1cm]{Figure/robot-clipart-xl}};


\end{tikzpicture}

